Traffic Scenario Logic: A Spatial-Temporal Logic for Modeling and Reasoning of Urban Traffic Scenarios

Formal representations of traffic scenarios can be used to generate test cases for the safety verification of autonomous driving. However, most existing methods are limited to highway or highly simplified intersection scenarios due to the intricacy and diversity of traffic scenarios. In response, we propose Traffic Scenario Logic (TSL), which is a spatial-temporal logic designed for modeling and reasoning of urban pedestrian-free traffic scenarios. TSL provides a formal representation of the urban road network that can be derived from OpenDRIVE, i.e., the de facto industry standard of high-definition maps for autonomous driving, enabling the representation of a broad range of traffic scenarios without discretization approximations. We implemented the reasoning of TSL using Telingo, i.e., a solver for temporal programs based on Answer Set Programming, and tested it on different urban road layouts. Demonstrations show the effectiveness of TSL in test scenario generation and its potential value in areas like decision-making and control verification of autonomous driving. The code for TSL reasoning has been open-sourced.

==> chapters/preliminary.tex <==
\section{Preliminary}

In this section, we provide a brief introduction to the road coordinate system and OpenDRIVE map format, the de facto industry standard of HD maps for autonomous driving.

The road coordinate system, also known as the Frenet frame, describes motions on a continuous differentiable curve in 3-dimensional Euclidean space.
Since the slope angle and superelevation of a road in the vertical direction are commonly small, what is used for road coordinate description is mostly a 2-dimensional version.
The road coordinate system is composed of the $S$ axis along the direction of the road reference line (generally the road centerline) and its orthogonal $D$ axis (also referred to as the $L$ or $T$ axis in some literature).
The coordinates of a point on the road are determined by its accumulated distance $s$ along the road reference line from the start point and the distance $d$ between the point and its projection onto the reference line.
With the road coordinate system, we can mitigate the influence of road curvature and uniformly describe the vehicle's position on the road.

\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
    %uncomment if require: \path (0,286); %set diagram left start at 0, and has height of 286
    
    %Curve Lines [id:da3077209292497054] 
    \draw [line width=1.25]    (40,86) .. controls (113.33,13) and (219.33,124) .. (307.33,59) ;
    %Curve Lines [id:da6172457271964737] 
    \draw [line width=1.25]    (73,118) .. controls (123.33,65) and (243.33,167) .. (329.33,97) ;
    %Shape: Axis 2D [id:dp33968796125420586] 
    \draw  (165.36,108.71) -- (261.95,134.57)(198.29,24.36) -- (172.43,120.95) (256.48,127.93) -- (261.95,134.57) -- (253.9,137.59) (191.65,29.82) -- (198.29,24.36) -- (201.31,32.41)  ;
    %Curve Lines [id:da8298552425485257] 
    \draw [line width=1.25]    (101,159) .. controls (144.33,116) and (283.33,217) .. (357.33,133) ;
    %Shape: Circle [id:dp018709589092698264] 
    \draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (176,86.5) .. controls (176,83.46) and (178.46,81) .. (181.5,81) .. controls (184.54,81) and (187,83.46) .. (187,86.5) .. controls (187,89.54) and (184.54,92) .. (181.5,92) .. controls (178.46,92) and (176,89.54) .. (176,86.5) -- cycle ;
    %Straight Lines [id:da26469262190958753] 
    \draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]    (181.5,86.5) -- (175.02,111.29) ;
    %Curve Lines [id:da8420101772446482] 
    \draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=3]    (73,118) .. controls (95.33,97) and (121.33,99) .. (175.02,111.29) ;
    %Shape: Brace [id:dp2721712512829102] 
    \draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (185.33,112) .. controls (188.49,112.83) and (190.48,111.66) .. (191.3,108.5) -- (191.3,108.5) .. controls (192.48,103.99) and (194.65,102.15) .. (197.8,102.97) .. controls (194.65,102.15) and (193.66,99.48) .. (194.83,94.97)(194.3,97) -- (194.83,94.97) .. controls (195.66,91.82) and (194.49,89.83) .. (191.33,89) ;
    %Shape: Brace [id:dp8703027038342785] 
    \draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (75.33,126) .. controls (75.66,130.65) and (78.16,132.81) .. (82.81,132.48) -- (91.09,131.89) .. controls (97.74,131.42) and (101.23,133.51) .. (101.56,138.16) .. controls (101.23,133.51) and (104.38,130.94) .. (111.03,130.47)(108.04,130.68) -- (166.85,126.47) .. controls (171.5,126.14) and (173.66,123.64) .. (173.33,118.99) ;
    %Curve Lines [id:da22550567174632508] 
    \draw    (115.33,41) .. controls (144.58,50.75) and (156.72,78.56) .. (166.58,99.41) ;
    \draw [shift={(167.33,101)}, rotate = 244.54] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    
    % Text Node
    \draw (-20,103) node [anchor=north west][inner sep=0.75pt]   [align=right] {\begin{minipage}[lt]{45.82pt}\setlength\topsep{0pt}
    reference\\
    line
    \end{minipage}};
    % Text Node
    \draw (200,93.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$d$};
    % Text Node
    \draw (95,137) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$s$};
    % Text Node
    \draw (265,130.4) node [anchor=north west][inner sep=0.75pt]    {$S$};
    % Text Node
    \draw (192,5.4) node [anchor=north west][inner sep=0.75pt]    {$D$};
    % Text Node
    \draw (-30,33) node [anchor=north west][inner sep=0.75pt]   [align=left] {projection point};
    
    
    \end{tikzpicture}
    \caption{The road coordinate system. The coordinate of the red dot consists of its accumulated distance $s$ along the reference line and the distance $d$ to the projection point.}
    \label{fig:frenet-frame}
\end{figure}

OpenDRIVE\footnote{https://www.asam.net/standards/detail/opendrive/} is a standardized HD map file format for representing road networks, encapsulating information about road geometry, topology, traffic signs, etc.
Each road in an OpenDRIVE file consists of road segments with a specific number of lanes, as depicted in \autoref{fig:map-1}.
Junctions are used to connect the roads, creating a connecting road for each pair of connected lanes.
Due to its powerful representation capabilities, OpenDRIVE has become the most widely used HD map format in autonomous driving and simulators such as CARLA.

\begin{figure}[htbp]
    \centering 

    \subcaptionbox{OpenDRIVE map\label{fig:map-1}}{
    
    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=0.8]
    %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

    %Straight Lines [id:da967142401281649] 
    \draw [line width=1.5]    (50.67,70) -- (150,70) ;
    %Straight Lines [id:da5055305466458728] 
    \draw [line width=1.5]    (50,100) -- (150,100) ;
    %Straight Lines [id:da8160940605869746] 
    \draw [line width=1.5]    (50,130) -- (150,130) ;
    %Straight Lines [id:da7317511960563905] 
    \draw [line width=1.5]    (150,70) -- (150,130) ;
    %Straight Lines [id:da45002668562290293] 
    \draw [line width=1.5]    (270.67,70) -- (370,70) ;
    %Straight Lines [id:da1177870336895972] 
    \draw [line width=1.5]    (270,100) -- (370,100) ;
    %Straight Lines [id:da32056930615245416] 
    \draw [line width=1.5]    (270,130) -- (370,130) ;
    %Straight Lines [id:da058212192178462185] 
    \draw [line width=1.5]    (270.67,70) -- (270.67,130) ;
    %Straight Lines [id:da5240425416457759] 
    \draw [line width=1.5]    (240,160) -- (240,220) ;
    %Straight Lines [id:da18587131693225967] 
    \draw [line width=1.5]    (210,160) -- (210,220) ;
    %Straight Lines [id:da6395639227862877] 
    \draw [line width=1.5]    (180,160) -- (240,160) ;
    %Straight Lines [id:da35679970284453133] 
    \draw [line width=1.5]    (180,160) -- (180,220) ;
    %Straight Lines [id:da9597111175113964] 
    \draw    (150,70) -- (270,70) ;
    %Straight Lines [id:da5504713120631828] 
    \draw    (150,100) -- (270,100) ;
    %Straight Lines [id:da7102890378545224] 
    \draw    (150,130) -- (270,130) ;
    %Curve Lines [id:da3052243908443546] 
    \draw    (150,130) .. controls (169.33,130.17) and (181.33,141.17) .. (180,160) ;
    %Curve Lines [id:da1225776764594928] 
    \draw    (150,100) .. controls (190.33,100.17) and (211.33,122.17) .. (210,160) ;
    %Curve Lines [id:da2192208235978672] 
    \draw    (150,70) .. controls (210.33,69.17) and (241.33,98.17) .. (240,160) ;
    %Curve Lines [id:da8064804787528341] 
    \draw    (180,160) .. controls (180.33,90.17) and (211.33,69.17) .. (270,70) ;
    %Curve Lines [id:da6635376589507567] 
    \draw    (210,160) .. controls (210.33,120.17) and (230.33,99.17) .. (270,100) ;
    %Curve Lines [id:da1829476270969428] 
    \draw    (240,160) .. controls (240.33,140.17) and (251.33,129.17) .. (270.67,130) ;
    %Straight Lines [id:da5653600443395197] 
    \draw    (60,115) -- (98,115) ;
    \draw [shift={(100,115)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6226310755386157] 
    \draw    (320,115) -- (358,115) ;
    \draw [shift={(360,115)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da4936071333732175] 
    \draw    (225,210) -- (225,182) ;
    \draw [shift={(225,180)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da09017216880653867] 
    \draw    (100,85) -- (62,85) ;
    \draw [shift={(60,85)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da2642460014300496] 
    \draw    (360,85) -- (322,85) ;
    \draw [shift={(320,85)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da9719836720301029] 
    \draw    (195,180) -- (195,208) ;
    \draw [shift={(195,210)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Shape: Polygon [id:ds0359235831457303] 
    \draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.18 ] (270,150) -- (260,160) -- (160,160) -- (150,150) -- (150.67,50) -- (270,50) -- cycle ;
    
    % Text Node
    \draw (182,52) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {Junction};
    
    
    \end{tikzpicture}
    }

    \subcaptionbox{Topology abstraction.\label{fig:map-2}}{

    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=0.8]
    %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
    
    %Straight Lines [id:da5143151436924736] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (75.67,65.5) -- (175,65.5) ;
    %Straight Lines [id:da26793915811285673] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (75,95.5) -- (175,95.5) ;
    %Straight Lines [id:da6781113644344019] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (75,125.5) -- (175,125.5) ;
    %Straight Lines [id:da2552253791820507] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (175,65.5) -- (175,125.5) ;
    %Straight Lines [id:da4029130395137974] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (295.67,65.5) -- (395,65.5) ;
    %Straight Lines [id:da9581029206548575] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (295,95.5) -- (395,95.5) ;
    %Straight Lines [id:da29232786256535825] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (295,125.5) -- (395,125.5) ;
    %Straight Lines [id:da296802634564032] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (295.67,65.5) -- (295.67,125.5) ;
    %Straight Lines [id:da8994823579756077] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (265,155.5) -- (265,215.5) ;
    %Straight Lines [id:da8055541978822163] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (235,155.5) -- (235,215.5) ;
    %Straight Lines [id:da42363909075946204] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (205,155.5) -- (265,155.5) ;
    %Straight Lines [id:da14935213534215896] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=1.5]    (205,155.5) -- (205,215.5) ;
    %Straight Lines [id:da3611078365826792] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,65.5) -- (295,65.5) ;
    %Straight Lines [id:da8593675651170494] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,95.5) -- (295,95.5) ;
    %Straight Lines [id:da8100204806902414] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,125.5) -- (295,125.5) ;
    %Curve Lines [id:da41825264677859253] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,125.5) .. controls (194.33,125.67) and (206.33,136.67) .. (205,155.5) ;
    %Curve Lines [id:da9633796601251912] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,95.5) .. controls (215.33,95.67) and (236.33,117.67) .. (235,155.5) ;
    %Curve Lines [id:da10619551251416004] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (175,65.5) .. controls (235.33,64.67) and (266.33,93.67) .. (265,155.5) ;
    %Curve Lines [id:da8257642085274246] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (205,155.5) .. controls (205.33,85.67) and (236.33,64.67) .. (295,65.5) ;
    %Curve Lines [id:da5097974887041512] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (235,155.5) .. controls (235.33,115.67) and (255.33,94.67) .. (295,95.5) ;
    %Curve Lines [id:da24456327384681398] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (265,155.5) .. controls (265.33,135.67) and (276.33,124.67) .. (295.67,125.5) ;
    %Straight Lines [id:da23099524119512616] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (85,110.5) -- (123,110.5) ;
    \draw [shift={(125,110.5)}, rotate = 180] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da11785687300095438] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (345,110.5) -- (383,110.5) ;
    \draw [shift={(385,110.5)}, rotate = 180] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da4276626447426761] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (250,205.5) -- (250,177.5) ;
    \draw [shift={(250,175.5)}, rotate = 90] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da6517931025214432] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (125,80.5) -- (87,80.5) ;
    \draw [shift={(85,80.5)}, rotate = 360] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da34003335313915417] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (385,80.5) -- (347,80.5) ;
    \draw [shift={(345,80.5)}, rotate = 360] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    %Straight Lines [id:da9567654777222088] 
    \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ]   (220,175.5) -- (220,203.5) ;
    \draw [shift={(220,205.5)}, rotate = 270] [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.25 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
    
    %Straight Lines [id:da8358098142485708] 
    \draw    (80,80) -- (180,80) ;
    %Straight Lines [id:da11047987994733877] 
    \draw    (80,110) -- (180,110) ;
    %Straight Lines [id:da7014146420120053] 
    \draw    (300,80) -- (390.33,80) ;
    %Straight Lines [id:da5875530511515841] 
    \draw    (300,110) -- (390.33,110) ;
    %Straight Lines [id:da4134369251280161] 
    \draw    (220,160) -- (220,210.5) ;
    %Straight Lines [id:da0267807214504987] 
    \draw    (250,160) -- (250,210.17) ;
    %Straight Lines [id:da17661538823907397] 
    \draw    (180,80) -- (300,80) ;
    %Straight Lines [id:da9726345329894823] 
    \draw    (180,110) -- (300,110) ;
    %Curve Lines [id:da7229356080535831] 
    \draw    (180,80) .. controls (230,80.17) and (250,98.08) .. (250,160) ;
    %Curve Lines [id:da5502084257141762] 
    \draw    (180,110) .. controls (209.33,110.17) and (219.33,141.17) .. (220,160) ;
    %Curve Lines [id:da7496010708527661] 
    \draw    (250,160) .. controls (250.33,141.17) and (270.33,110.17) .. (300,110) ;
    %Curve Lines [id:da5361548338528783] 
    \draw    (220,160) .. controls (220,95.58) and (240.67,79.83) .. (300,80) ;
    %Flowchart: Decision [id:dp8176140673087307] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (175,75) -- (180,80) -- (175,85) -- (170,80) -- cycle ;
    %Flowchart: Decision [id:dp13520318017042476] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (175,105) -- (180,110) -- (175,115) -- (170,110) -- cycle ;
    %Flowchart: Decision [id:dp46000772997083894] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (295,75) -- (300,80) -- (295,85) -- (290,80) -- cycle ;
    %Flowchart: Decision [id:dp7530109396225653] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (295,105) -- (300,110) -- (295,115) -- (290,110) -- cycle ;
    %Flowchart: Decision [id:dp5753240763704699] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (220,150) -- (225,155) -- (220,160) -- (215,155) -- cycle ;
    %Flowchart: Decision [id:dp9546628780258557] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (250,150) -- (255,155) -- (250,160) -- (245,155) -- cycle ;
    %Flowchart: Summing Junction [id:dp17556873516622473] 
    \draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (236.67,110.33) .. controls (236.67,107.57) and (238.91,105.33) .. (241.67,105.33) .. controls (244.43,105.33) and (246.67,107.57) .. (246.67,110.33) .. controls (246.67,113.09) and (244.43,115.33) .. (241.67,115.33) .. controls (238.91,115.33) and (236.67,113.09) .. (236.67,110.33) -- cycle ; \draw   (238.13,106.8) -- (245.2,113.87) ; \draw   (245.2,106.8) -- (238.13,113.87) ;
    %Flowchart: Summing Junction [id:dp7659840716537447] 
    \draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (230,100.5) .. controls (230,97.74) and (232.24,95.5) .. (235,95.5) .. controls (237.76,95.5) and (240,97.74) .. (240,100.5) .. controls (240,103.26) and (237.76,105.5) .. (235,105.5) .. controls (232.24,105.5) and (230,103.26) .. (230,100.5) -- cycle ; \draw   (231.46,96.96) -- (238.54,104.04) ; \draw   (238.54,96.96) -- (231.46,104.04) ;
    %Flowchart: Summing Junction [id:dp4813615772280697] 
    \draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (223.67,109.93) .. controls (223.67,107.17) and (225.91,104.93) .. (228.67,104.93) .. controls (231.43,104.93) and (233.67,107.17) .. (233.67,109.93) .. controls (233.67,112.69) and (231.43,114.93) .. (228.67,114.93) .. controls (225.91,114.93) and (223.67,112.69) .. (223.67,109.93) -- cycle ; \draw   (225.13,106.4) -- (232.2,113.47) ; \draw   (232.2,106.4) -- (225.13,113.47) ;
    %Flowchart: Decision [id:dp7441659486943573] 
    \draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (87,160) -- (92,165) -- (87,170) -- (82,165) -- cycle ;
    %Flowchart: Summing Junction [id:dp5122682523860609] 
    \draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (82,185) .. controls (82,182.24) and (84.24,180) .. (87,180) .. controls (89.76,180) and (92,182.24) .. (92,185) .. controls (92,187.76) and (89.76,190) .. (87,190) .. controls (84.24,190) and (82,187.76) .. (82,185) -- cycle ; \draw   (83.46,181.46) -- (90.54,188.54) ; \draw   (90.54,181.46) -- (83.46,188.54) ;
    
    % Text Node
    \draw (97.88,165) node [anchor=west] [inner sep=0.75pt]  [font=\scriptsize] [align=left] {connect point};
    % Text Node
    \draw (97.88,185) node [anchor=west] [inner sep=0.75pt]  [font=\scriptsize] [align=left] {intersect point};
    % Text Node
    \draw (361,71) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l1};
    % Text Node
    \draw (361,101) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l2};
    % Text Node
    \draw (91,71) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l3};
    % Text Node
    \draw (91,101) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l4};
    % Text Node
    \draw (221,202) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l5};
    % Text Node
    \draw (251,202) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l6};
    % Text Node
    \draw (226,71) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l13};
    % Text Node
    \draw (261,101) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {l42};
    % Text Node
    \draw (200.41,122.07) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-48.58] [align=left] {l45};
    % Text Node
    \draw (259.81,137.04) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-303.2] [align=left] {l62};
    % Text Node
    \draw (208.76,86.02) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-25.09] [align=left] {l63};
    % Text Node
    \draw (222.07,143.09) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-274.56] [align=left] {l15};
    % Text Node
    \draw (291,67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n1};
    % Text Node
    \draw (291,97) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n2};
    % Text Node
    \draw (169,67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n3};
    % Text Node
    \draw (171,97) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n4};
    % Text Node
    \draw (201,152) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n5};
    % Text Node
    \draw (259,152) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {n6};
    % Text Node
    \draw (243,94.5) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {x1};
    % Text Node
    \draw (211,112) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {x2};
    % Text Node
    \draw (246,112) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {x3};
    
    
    \end{tikzpicture}

    }

    \caption{A typical T-intersection. Six connecting roads link three 2-lane roads in the junction area.}
    \label{fig:map}
\end{figure}


